Publicly-Detectable Watermarking for Language Models

We present a publicly-detectable watermarking scheme for LMs: the detection algorithm contains no secret information, and it is executable by anyone. We embed a publicly-verifiable cryptographic signature into LM output using rejection sampling and prove that this produces unforgeable and distortion-free (i.e., undetectable without access to the public key) text output. We make use of error-correction to overcome periods of low entropy, a barrier for all prior watermarking schemes. We implement our scheme and find that our formal claims are met in practice.

==> notes.tex <==
overview diagram flow:
1. LM provider genrates sk and pk. keeps sk secret.
2. LM provider publicizes pk (e.g., uploads it to a public bulletin board)
3. User queries the LM with a prompt.
4. LM provider replies to the query with a text response.
5. User retrieves the LM providers pk from the bulletin board, and runs Detect\_pk(text) to determine if the text really came from LM provider or not.

- rewrite intro to focus on strengths: cryptographic correctness/soundness and trustlessness
- add christ et al new paper to future work

old intro:

Generative AI (GenAI) technologies, such as large language models (LLMs) and diffusion models, have impressive capabilities. 
These capabilities include in-context learning, code completion, text-to-image generation, and document and code chat.
However, GenAI technologies are also being used for nefarious purposes (e.g., generating fake tweets, generating attacks,  and harmful prose).   
To protect against such use cases, a large body of work has focused on detecting AI-generated content~\citep{lavergne2008detecting,beresneva2016computer,gehrmann2019gltr,zellers2019defending,mitchell2023detectgpt,gptzero,openaidetector}. 
The problem is as follows: given content $c$, is $c$ generated by some specific GenAI technique, e.g., GPT-4~\citep{openai2023gpt4}, Gemini~\citep{gemini}, or Stable Diffusion~\citep{rombach2022high}? In other words, informally speaking, we want a ``GenAI Turing Test.'' 

At present, the main approach when trying to detect AI-generated text is to train yet another AI model to perform the detection~\citep{zellers2019defending,mitchell2023detectgpt,gptzero,openaidetector}.
This method makes a critical assumption: that AI-generated text has embedded features that are identifiable by AI.
%that AI-generated text has features embedded within it that AI can identify.
The key problem with this assumption is that generative models are explicitly designed to produce realistic content that is difficult to distinguish from natural content (generated by a human or nature). 
As a result, any ``black-box'' detection scheme will suffer from high false positive and/or false negative rates as generative models improve.
Available detectors such as GPTZero~\citep{gptzero} have no guarantee of correctness---e.g., the authors state outright that detection results from their tool should not be used to punish students.

To circumvent this fundamental issue, a recent line of work~\citep{neurocryptography,kirchenbauer2023watermark,christ2023undetectable,kuditipudi2023robust} has taken a different approach to detecting AI content.
By embedding a watermark into content at generation-time, they are able to meet a stronger detection criteria. 
Watermarking techniques alter the generation process to embed some ``secret'' in the generated content. 
Such a secret is embedded into the content in a way that one who knows the secret can detect it, so long as the generated content is not altered significantly. 
In particular, the cryptographic approach of~\citet{christ2023undetectable} achieves formal notions of completeness (any watermarked text will be detected), soundness (one cannot watermark a text without knowing the secret), and distortion-freeness (watermarking does not change the output distribution).

In summary, these watermarking techniques embed a ``signal'' in the output of the generative model, where the signal depends on a secret key. 
Note that detecting whether a piece of text is watermarked does not require access to the model. 
Once a text $t$ is received, one can check whether it was watermarked or not using the secret key.
Thus, the secret key is used for both embedding and detecting the watermark. 

The aforementioned watermarking approaches have one problem in common: the generative model and the detector both need to know the secret key. 
% That is, the detector cannot detect AI-generated content unless it knows the secret that was embedded in the content. 
This is acceptable in scenarios where the entity trying to detect the watermark is the same entity generating the content.
For example, an entity that provides a chat API may be able to provide a detection API as well. 
However, such a setup has limitations:
\begin{enumerate}
    \item \textbf{Lack of privacy:} The entity who wants to check the integrity of the content might not be willing to share it with the detector. For example, one looking to identify whether their medical records are AI-generated may not want to share the records themselves.
    \item \textbf{Conflict of interest:} The entity providing the detection API might not be trusted in certain cases. 
    For instance, consider a case where the entity is accused of generating a certain inappropriate text and is brought to a court of law. 
    It is not reasonable to ask the same entity to tell whether the text is watermarked.
    % \item \textbf{Inefficiency:} Providing a detection API is costly.
\end{enumerate}

One solution could be sharing the secret with the world so everyone can run the detection. 
However, this raises another important problem: anyone can now embed the secret to any content, AI-generated or not. 
This would not be acceptable because the watermarking is subject to denial of service attacks. 
An attacker can create masses of watermarked content that is not AI-generated to undermine the dependability of the detector. 
Consider the effect on one of the main applications of watermarking: an entity may want to use the watermark as a signature for their content. Such signatures are useful when (a) the generated content needs to come with proof of a credible generator, and (b) the entity needs to refute an accusation about a generated content; i.e., it should not be accountable for a content without its watermark. This application is rendered impossible in a world with availability attacks.
% It also defeats one of the main applications of watermarking, in which an entity might want to use the watermark as a signature for their content. 
% This would be useful when the generated content needs to come with proof that it is generated by a credible source. 
% Such signatures are also useful to refute any accusations about a generated content; an entity would not be accountable for a content if it does not have their signature (watermark). 

In this paper, we aim to solve the aforementioned problems for LLMs that produce text. We ask:
\begin{quote}
    \centering
    \textit{Is it possible to construct a {\em publicly-detectable} watermarking scheme?}
\end{quote}
We find that the answer is yes: we construct a publicly-detectable scheme that provably resolves the trust issue---users can cryptographically verify the presence of a watermark.
Further, they have a guarantee that the only entity capable of embedding the watermark is the model provider, resolving the privacy and conflict of interest issues above.
We state the properties for public detectability below:
\begin{enumerate}
    \item \textbf{Security:} To guarantee a user is convinced that a watermark is detected, the watermarking scheme must be cryptographic in the sense that false positives are ``essentially impossible'' in a rigorous mathematical sense as opposed to empirical validation---it should be impossible for any probabilistic polynomial-time (PPT) adversary to attack the scheme.
    \item \textbf{Weak robustness:} It is likely that text obtained from LMs is modified---to some extent---before publication.
    The watermark detector should be robust in the sense that it can still detect a watermark as long as the cryptographic signature is still embedded in the text.
    Prior work in the secret key setting aimed for \textit{strong} robustness where detection should be possible even if the LM output has changed substantially but text semantics are preserved. Strong robustness has since been shown to be impossible in the general case~\citep{zhang2023watermarks}.
    \item \textbf{Distortion-freeness:} The watermarking scheme should not degrade the quality of the LM output. No PPT adversary should be able to distinguish between watermarked and non-watermarked text.
    \item \textbf{Model agnosticity:} The watermarking scheme should use the model as a black box, i.e., it should not rely on any specific model weights or configurations.
    \item \textbf{Public verifiablity:} Without access to the model weights or secret material of the watermarking scheme, the detector should be able to determine whether a candidate text is watermarked.
\end{enumerate}

% ----------------------------------------------------------------------

\begin{algorithm}[H]
\caption{Private Watermark Generator (Old)}\label{alg:generate}
\begin{algorithmic}[1]
\STATE {\bfseries input:} $\sk$, $n$, $\ell$, $\lambda_c$, $\beta$, $a_{\mathrm{max}}$, $\gamma_{\mathrm{max}}$, $\prompt$ 
    \STATE $\tokens \gets \epsilon$ \COMMENT{Initialize output tokens}
    \WHILE[While there are fewer less than $n$ tokens]{$\abs{\tokens} + \ell \cdot \lambda_c < n$}\alglinelabel{line:wrapper} 
        \STATE $\tokens \gets \tokens \parallel \genmodel_\ell(\prompt, \tokens)$\COMMENT{Sample $\ell$ tokens from plain model and append to output} \alglinelabel{line:get_message}
        \STATE $\boldsymbol{\sigma}\gets \Sign_\sk(\hash_1(\tokens[-\ell:]))$ \COMMENT{Mask the codeword with another hash} \alglinelabel{line:hash_and_sign_0}
        \STATE $\mathbf{c} \gets \hash_2(\tokens[-\ell:]) \oplus \encode_\gamma(\boldsymbol{\sigma})$ \COMMENT{ECC} \alglinelabel{line:hash_and_sign}
        \STATE $\mathbf{m}, \mathbf{c}_\mathsf{prev} \gets \epsilon, \epsilon$ \COMMENT{Initialize } \alglinelabel{}
        \STATE $\gamma \gets 0$
        \WHILE {$\mathbf{c} \neq \epsilon$}
            \STATE $c, \mathbf{c} \gets \mathbf{c}[0:\beta], \mathbf{c}[\beta:]$ 
            % \mingyuan{Since you are embedding multiple bits, lets use some symbol here. maybe $\mathbf{c}[0:\beta], \mathbf{c}[\beta:]$. I used $\beta$ in the text}
            \STATE $a \gets 0$
            \STATE $\mathbf{x}_{\mathrm{best}}, d_{\mathrm{best}} \gets \epsilon, \infty$
            \REPEAT \alglinelabel{line:embed_start}
                \STATE $\mathbf{x} \gets \genmodel_\ell(\prompt, \tokens)$
                \STATE $a \gets a + 1$
                \STATE $d \gets \mathsf{Hamming}(\hash_1(\mathbf{m} \parallel \mathbf{x} \parallel \mathbf{c}_\mathsf{prev}), c)$
                \IF {$d < d_{\mathrm{best}}$}
                    \STATE $d_{\mathrm{best}}, \mathbf{x}_{\mathrm{best}} \gets d, \mathbf{x}$
                \ENDIF 
                \IF {
                $(a > a_{\mathrm{max}} \ \land \ \gamma < \gamma_{\mathrm{max}})$
                }
                    \STATE $\mathbf{x} \gets \mathbf{x}_{\mathrm{best}}$
                    \STATE $\gamma \gets \gamma + 1$
                    \STATE {\bf break}
                \ENDIF
            \UNTIL {$\hash_1(\mathbf{m} \parallel \mathbf{x} \parallel \mathbf{c}_\mathsf{prev}) = c$}
            \alglinelabel{line:embed_end} 
            \STATE $\mathbf{m} \gets \mathbf{m} \parallel \mathbf{x}$
            \STATE $\tokens \gets \tokens \parallel \mathbf{x}$
            \STATE $\mathbf{c}_\mathsf{prev} \gets \mathbf{c}_\mathsf{prev} \parallel c$
        \ENDWHILE
    \ENDWHILE
    \IF {$\abs{\tokens} < n$}
        \STATE $\tokens \gets \tokens \parallel \genmodel_{n - \abs{\tokens}}(\prompt, \tokens)$
    \ENDIF
    \STATE {\bfseries output:} $\tokens$
\end{algorithmic}
\end{algorithm}
